Efficient Neural Network Implementation with Quadratic Neuron

Previous works proved that the combination of the linear neuron network with nonlinear activation functions (e.g. ReLu) can achieve nonlinear function approximation. However, simply widening or deepening the network structure will introduce some training problems. In this work, we are aiming to build a comprehensive second-order CNN implementation framework that includes neuron/network design and system deployment optimization.

==> 0_abstract.tex <==
\begin{abstract}
	Recently, the machine learning technologies have been widely used in cognitive applications such as Automatic Speech Recognition (ASR) and Image Recognition (IR).
	Unfortunately, these techniques have been massively used in unauthorized audio/image data analysis, causing serious privacy leakage.
	%analyze massive audio/image data without authorization, which will cause serious privacy information leakage.
To address this issue, we propose \textit{HAMPER} in this work, which is a data encryption framework that protects the audio/image data from unauthorized ASR/IR analysis.
To address this issue, we propose \textit{HAMPER} in this work, which is a data encryption framework that protects the audio/image data from unauthorized ASR/IR analysis.
	Experiment results show that, \textit{HAMPER} can effectively perturb the unauthorized ASR/IR analysis with 85\% Word-Error-Rate (WER) and 83\% Image-Error-Rate (IER) respectively.
	Also, \textit{HAMPER} achieves faster processing speed with 1.5$\times$ speedup for image encryption and even 26$\times$ in audio, comparing to the state-of-the-art methods.
	Moreover, \textit{HAMPER} achieves strong transferability and configures adversarial examples with desired attributes for better scenario adaptation.
\end{abstract}

